Schema for In-Context Learning

In-Context Learning (ICL) enables transformer-based language models to adapt to new tasks by conditioning on demonstration examples. However, traditional example-driven in-context learning lacks explicit modules for knowledge retrieval and transfer at the abstraction level. Inspired by cognitive science, specifically schema theory, which holds that humans interpret new information by activating pre-existing mental frameworks (schemas) to structure understanding, we introduce Schema-Activated In-Context Learning (SA-ICL). This framework extracts the representation of the building blocks of cognition for the reasoning process instilled from prior examples, creating an abstracted schema, a lightweight, structured template of key inferential steps and their relationships, which is then used to augment a model's reasoning process when presented with a novel question. We demonstrate that a broad range of large language models (LLMs) lack the capacity to form and utilize internal schema-based learning representations implicitly, but instead benefit significantly from explicit schema-based scaffolding. Across chemistry and physics questions from the GPQA dataset, our experiments show that SA-ICL consistently boosts performance, up to 36.19 percent, when the single demonstration example is of high quality, which simultaneously reduces reliance on the number of demonstrations and enhances interpretability. Schema-Activated In-Context Learning not only bridges disparate ICL strategies ranging from pattern priming to Chain-of-Thought prompting, but also paves a new path for enhancing human-like reasoning in LLMs.

==> latex/sections/Results/extra.tex <==
\begin{table}[h!]
\centering
\small
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.1}
\caption{Performances of {\sysname}, {\oneshot}, One-Shot with Reasoning and 5-Shots on MedXpertQA, MMLU, and CommonSenseQA questions. Note that for the MMLU questions were the original MMLU questions included in the MMLU-Pro dataset, for MedXpertQA, we were using the Skeletal questions, for CommonSenseQA, we randomly picked up 200 questions from the validation subset.}
\label{tab:benchmark_comparison}
\begin{tabular}{p{0.3\columnwidth} p{0.3\columnwidth} c}
\toprule
\textbf{Dataset} & \textbf{Method} & \textbf{Accuracy} \\
\midrule
\multirow{4}{*}{\textbf{MMLU CollegeMath}} 
 & SA-ICL & \textbf{0.7973} \\
 & One-Shot & 0.6216 \\
 & One-Shot + Reasoning & 0.7162 \\
 & 5-Shots & 0.7027 \\
\midrule
\multirow{4}{*}{\textbf{MedXpertQA}} 
 & SA-ICL & \textbf{0.7342} \\
 & One-Shot & 0.6034 \\
 & One-Shot + Reasoning & 0.6667 \\
 & 5-Shots & 0.7027 \\
\midrule
\multirow{4}{*}{\textbf{CommonSense}} 
 & SA-ICL & \textbf{0.9200} \\
 & One-Shot & 0.9000 \\
 & One-Shot + Reasoning & 0.8400 \\
 & 5-Shots & 0.8800 \\
\bottomrule
\end{tabular}
\end{table}


==> latex/sections/Results/name.tex <==
\begin{table}[h!]
\centering
\small
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.1}
\caption{Performance Comparison Across Benchmarks and Methods}
\begin{tabular}{l l c}
\toprule
\textbf{Dataset} & \textbf{Method} & \textbf{Accuracy} \\
\midrule
\multirow{4}{*}{\textbf{MMLUCollegeMath}} 
 & SA-ICL & \textbf{79.73\%} \\
 & One-Shot & 62.16\% \\
 & One-Shot with Reasoning & 71.62\% \\
 & 5-Shots & 70.27\% \\
\midrule
\multirow{4}{*}{\textbf{MedXpertQA}} 
 & SA-ICL & \textbf{73.42\%} \\
 & One-Shot & 60.34\% \\
 & One-Shot with Reasoning & 66.67\% \\
 & 5-Shots & 70.27\% \\
\midrule
\multirow{4}{*}{\textbf{CommonSense}} 
 & SA-ICL & \textbf{92\%} \\
 & One-Shot & 90\% \\
 & One-Shot with Reasoning & 84\% \\
 & 5-Shots & 88\% \\
\bottomrule
\end{tabular}
\end{table}


==> latex/sections/Results/pvalue-overall.tex <==
\begin{table}[h]
    \centering
    \caption{Performance Impact Analysis}
    \label{tab:p_value_overall}
    % \resizebox{\columnwidth}{!} scales the table to the width of the text column
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{l c c c l}
            \toprule
            \textbf{Metric} & \textbf{Baseline} & \textbf{Final} & \textbf{Change ($\Delta$)} & \textbf{$p$-value} \\
            \midrule
            Reasoning Impact & 43.4\% & 43.6\% & +0.2\% & 0.7637 (ns) \\
            Schema Impact    & 43.6\% & 48.7\% & +5.1\% & 0.0000 (***) \\
            \bottomrule
        \end{tabular}%
    }
\end{table}

==> latex/sections/Results/table_backup.tex <==
\begin{table}[h!]
\label{tab:full_results}
\small
\centering
\caption{Performances of {\sysname} and {\oneshot} on Chemistry and Physics questions. For Chemistry, the improvement is up to \textbf{39.67\%}, \textbf{34.88\%} for Physics. On average, the improvement in Chemistry is \textbf{9.81\%}, \textbf{12.91\%} for Physics. All values in table were rounded up to the third decimal.}
\label{tab:model-comparison}

% Subtable for Chemistry
\begin{subtable}{\textwidth}
\centering
\caption{Chemistry Results}
\label{tab:chemistry-sub-comparison}
\begin{tabular}{@{}ll|ccc|ccc@{}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Synthetic Similarity} & \multicolumn{3}{c}{Latent Similarity} \\
 &  & {\same} & {\similar} & {\different} & High & Medium & Low \\
\midrule
\multirow{2}{*}{Qwen-3} & {\sysname} & \textbf{0.763}  & \textbf{0.376}  & 0.301 & 0.667  & \textbf{0.613} & 0.516 \\
 & {\oneshot} & 0.581  & 0.301  & 0.301 & \textbf{0.688}  & 0.581 & \textbf{0.624} \\
\midrule
\multirow{2}{*}{Llama-3.1} & {\sysname} & \textbf{0.892}  & \textbf{0.430}  & \textbf{0.387} & \textbf{0.753}  & \textbf{0.538}  & 0.376 \\
 & {\oneshot} & 0.495  & 0.366  & 0.366 & 0.441  & 0.441  & \textbf{0.473} \\
\midrule
\multirow{2}{*}{GPT-4o Mini} & {\sysname} & \textbf{0.946}  & \textbf{0.462}  & \textbf{0.366} & \textbf{0.839}  & 0.538  & 0.441 \\
 & {\oneshot} & 0.688  & 0.366  & 0.323 & 0.667  & \textbf{0.624}  & \textbf{0.613} \\
\midrule
\multirow{2}{*}{GPT-4o} & {\sysname} & \textbf{0.925}  & 0.516  & \textbf{0.419} & \textbf{0.774}  & \textbf{0.796}  & \textbf{0.828} \\
 & {\oneshot} & 0.656  & \textbf{0.559}  & 0.409 & 0.667  & 0.688  & 0.699 \\
\midrule
\multirow{2}{*}{Ministral} & {\sysname} & \textbf{0.882}  & \textbf{0.473}  & \textbf{0.376} & \textbf{0.785}  & \textbf{0.817}  & \textbf{0.860} \\
 & {\oneshot} & 0.731  & 0.376  & 0.280 & 0.677  & 0.656  & 0.656 \\
\midrule
\multirow{2}{*}{Gemini 1.5 Flash} & {\sysname} & \textbf{0.796}  & \textbf{0.333}  & \textbf{0.280} & \textbf{0.720}  & \textbf{0.581}  & \textbf{0.484} \\
 & {\oneshot} & 0.538  & 0.258  & 0.194 & 0.473  & 0.452  & 0.409 \\
\bottomrule
\end{tabular}
\end{subtable}

\vspace{1em} % Adds a bit of vertical space between the tables

% Subtable for Physics
\begin{subtable}{\textwidth}
\centering
\caption{Physics Results}
\label{tab:physics-sub-comparison}
\begin{tabular}{@{}ll|ccc|ccc@{}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Synthetic Similarity} & \multicolumn{3}{c}{Latent Similarity} \\
 &  & {\same} & {\similar} & {\different} & High & Medium & Low \\
\midrule
\multirow{2}{*}{Qwen-3} & {\sysname} & \textbf{0.756}  & 0.465  & 0.349 & \textbf{0.686}  & 0.523  & 0.535 \\
 & {\oneshot} & 0.616  & \textbf{0.477}  & \textbf{0.477} & 0.605  & \textbf{0.581}  & \textbf{0.581} \\
\midrule
\multirow{2}{*}{Llama-3.1} & {\sysname} & \textbf{0.814}  & \textbf{0.430}  & \textbf{0.407} & \textbf{0.744}  & \textbf{0.686}  & \textbf{0.558} \\
 & {\oneshot} & 0.512  & 0.314  & 0.372 & 0.465  & 0.395  & 0.547 \\
\midrule
\multirow{2}{*}{GPT-4o Mini} & {\sysname} & \textbf{0.977}  & \textbf{0.512}  & \textbf{0.523} & \textbf{0.872}  & \textbf{0.651}  & \textbf{0.570} \\
 & {\oneshot} & 0.628  & 0.372  & 0.372 & 0.593  & 0.593  & 0.547 \\
\midrule
\multirow{2}{*}{GPT-4o} & {\sysname} & \textbf{0.953}  & \textbf{0.663}  & \textbf{0.616} & \textbf{0.872}  & \textbf{0.907}  & \textbf{0.930} \\
 & {\oneshot} & 0.721  & 0.616  & 0.547 & 0.744  & 0.698  & 0.721 \\
\midrule
\multirow{2}{*}{Ministral} & {\sysname} & \textbf{0.930}  & \textbf{0.535}  & \textbf{0.488} & \textbf{0.849}  & \textbf{0.802}  & \textbf{0.791} \\
 & {\oneshot} & 0.802  & 0.372  & 0.256 & 0.663  & 0.721  & 0.686 \\
\midrule
\multirow{2}{*}{Gemini 1.5 Flash} & {\sysname} & \textbf{0.767}  & \textbf{0.407}  & \textbf{0.360} & \textbf{0.674}  & \textbf{0.651}  & \textbf{0.686} \\
 & {\oneshot} & 0.500  & 0.349  & 0.349 & 0.500  & 0.488  & 0.512 \\
\bottomrule
\end{tabular}
\end{subtable}

\end{table}

